Simulating Dynamic Tumor Contrast Enhancement in Breast MRI using Conditional Generative Adversarial Networks

This paper presents a method for virtual contrast enhancement in breast MRI, offering a promising non-invasive alternative to traditional contrast agent-based DCE-MRI acquisition. Using a conditional generative adversarial network, we predict DCE-MRI images, including jointly-generated sequences of multiple corresponding DCE-MRI timepoints, from non-contrast-enhanced MRIs, enabling tumor localization and characterization without the associated health risks. Furthermore, we qualitatively and quantitatively evaluate the synthetic DCE-MRI images, proposing a multi-metric Scaled Aggregate Measure (SAMe), assessing their utility in a tumor segmentation downstream task, and conclude with an analysis of the temporal patterns in multi-sequence DCE-MRI generation. Our approach demonstrates promising results in generating realistic and useful DCE-MRI sequences, highlighting the potential of virtual contrast enhancement for improving breast cancer diagnosis and treatment, particularly for patients where contrast agent administration is contraindicated.

==> tables/experiments_3_4.tex <==
\begin{table}[ht!]
\centering
\caption{Results for tumour segmentation test cases. In experiments \emph{3} data from both pre-contrast as well as post-contrast acquisitions is available enabling testing in the post-contrast domain.
Experiments \emph{4} demonstrate the benefit of synthetic post-contrast data in the scenario where segmentation models were trained in the post-contrast domain, but need to be applied to test subjects for which only pre-contrast data is available (e.g., due to allergy, pregnancy, or missing consent). %The reported Dice coefficient results are derived from the ensemble model over 5-fold cross-validation.
}
% \scriptsize
\vspace{2mm}
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{lc}
    \toprule
    Experiments \emph{3}. \small{Post-contrast training data and post-contrast test data available}  & Dice $\uparrow$ \\  \emph{train on:} & \emph{test on:} Real post-contrast  \\
    %\arrayrulecolor{black} \toprule
    \arrayrulecolor{light_grey} \toprule
    % 
    Real post-contrast (\emph{baseline 3}) & 0.790 \\
    Real post-contrast + syn post-contrast (augmentation)  & \textbf{0.797} \\
    Real post-contrast + real pre-contrast (augmentation) &  0.780 \\
    Real post-contrast + real pre-contrast + syn post-contrast (augmentation) & 0.770 \\
    Syn post-contrast & 0.687 \\
    % 
    %\arrayrulecolor{black} \bottomrule
    \arrayrulecolor{black} \toprule
     Experiments \emph{4}. \small{Domain shift: Post-contrast training data, but no post-contrast test data available}  & \\ \emph{train on:} &  \emph{test on:} Real pre-contrast   \\
    \arrayrulecolor{light_grey} \toprule
    % 
    Real post-contrast (\emph{baseline 4}) & 0.164 \\
    Real post-contrast + syn post-contrast (augmentation)  & 0.409 \\
    Syn post-contrast & \textbf{0.486} \\
    % 
    \arrayrulecolor{black} \bottomrule
\end{tabular}
}
\label{tab:experiments_3_4}
% \vspace{-2mm}
\end{table}
